Adversarial Personalized Ranking for Recommendation

Item recommendation is a personalized ranking task. To this end, many recommender systems optimize models with pairwise ranking objectives, such as the Bayesian Personalized Ranking (BPR). Using matrix Factorization (MF) --- the most widely used model in recommendation --- as a demonstration, we show that optimizing it with BPR leads to a recommender model that is not robust. In particular, we find that the resultant model is highly vulnerable to adversarial perturbations on its model parameters, which implies the possibly large error in generalization. To enhance the robustness of a recommender model and thus improve its generalization performance, we propose a new optimization framework, namely Adversarial Personalized Ranking (APR). In short, our APR enhances the pairwise ranking method BPR by performing adversarial training. It can be interpreted as playing a minimax game, where the minimization of the BPR objective function meanwhile defends an adversary, which adds adversarial perturbations on model parameters to maximize the BPR objective function. To illustrate how it works, we implement APR on MF by adding adversarial perturbations on the embedding vectors of users and items. Extensive experiments on three public real-world datasets demonstrate the effectiveness of APR --- by optimizing MF with APR, it outperforms BPR with a relative improvement of 11.2% on average and achieves state-of-the-art performance for item recommendation. Our implementation is available at: https://github.com/hexiangnan/adversarial_personalized_ranking.

==> 1_introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}
To address information overloading, recommender systems have been widely deployed in customer-oriented online services, such as E-commerce platforms, social media sites, news portals and so on. An effective recommendation solution not only can increase the traffic and profit for service providers, but also can help users find the items of interest more easily. In this work, we focus on the fundamental problem of item recommendation, which aims to generate a specific ranking list of items for each user. 

Due to the abundance of user feedback such ratings and purchases that can reflect a user's preference directly, research on recommendation has largely focused on mining the feedback data, known as collaborative filtering (CF). 
%SPACE
%There are several collaborative filtering models been developed to estimate a user's preference on an item from the feedback data, such as neighbor-based \cite{book:neighborCF}, graph-based \cite{Xiang:2010}, latent factor-based \cite{SVD++} and so on. 
Among the various CF methods, matrix factorization (MF)~\cite{koren2009matrix}
%SPACE
%, a special type of latent factor models, 
has been recognized as the basic yet most effective recommender model since several years.
Being a germ of representation learning \cite{RL_review}, MF represents each user and item as an embedding vector, and estimates the preference of a user on an item as the inner product of their embedding vectors. 
To learn MF, early work optimized a pointwise regression loss on user ratings~\cite{SVD++}. Later on, Rendle \etal~\cite{BPR} argued that item recommendation is a personalized ranking task, and such that, the optimization should be tailored for ranking rather than regression. They then proposed a pairwise learning method named \textit{Bayesian Personalized Ranking} (BPR), which optimizes a recommender model based on the relative preference of users over pairs of items. The pairwise optimization of BPR is particularly well suited for learning from implicit feedback, since it is natural to assume that the interacted items should be more preferred than the non-interacted ones for a user. Owing to its rationality and ease of optimization, BPR has been used in a wide variety of scenarios~\cite{FPMC,VBPR,Zhao:2014,Bi:2015,ACF,JRL,CKBE,LambdaFM} and plays a dominant role in optimizing recommender models. 

On the other hand, recent advance on adversarial machine learning~\cite{AML_2014,fawzi2016robustness,AML_2017} show that many well-behaved classifiers are actually very fragile and vulnerable to \textit{adversarial examples}, which are formed by applying small but intentionally perturbations to input examples from the dataset. A typical example can be found in Figure 1 of \cite{AML_2015}, which demonstrates that by adding small adversarial perturbations to an image of panda, a well-trained classier misclassified the image as a gibbon with a high confidence, whereas the effect of perturbations can hardly be perceived by human. This points to an inherent limitation of training a model on static labeled data only. To address the limitation, researchers then developed adversarial training methods that train a model to correctly classify the dynamically generated adversarial examples~\cite{AML_2015,AML_2017,moosavi2016universal}

While the inspiring progress of adversarial machine learning mainly concentrated on the computer vision domain where the adversarial examples can be understood intuitively, to date, there is no study about such adversarial phenomenon in IR domain. Although the core task in IR is ranking, we point out that many learning to rank (L2R) methods are essentially trained by optimizing a classification function, such as the pairwise L2R method BPR, among others~\cite{book_l2r}. Which means, it is likely that the underlying IR models also lack robustness and are vulnerable to certain kinds of ``adversarial examples''. This work aims to fill the research gap by exploring adversarial learning methods on item recommendation, an active topic of research in IR that concerns personalized ranking. 

Nevertheless, directly grafting the way of generating adversarial examples from the image domain is infeasible, since the inputs of recommender models are discrete ID features (\ie user ID and item ID) and it is meaningless to apply noises to ID features. To address this, we consider exploring the robustness of a recommender model at a deeper level --- at the level of its intrinsic model parameters rather than the extrinsic inputs. Using the MF model trained with BPR as a demonstration (we term this instantiation as MF-BPR), we investigate its robustness to perturbations on the embedding parameters. It is worth noting that MF-BPR is a highly competitive approach for item recommendation and has been used in many papers as the state-of-the-art baseline up until recently~\cite{fastMF,NCF,CML,LRML}. 
We find that MF-BPR is not robust and is vulnerable to adversarial perturbations on its parameters. This sheds light on the weakness of training recommender models with BPR, motivating us to develop adversarial training methods that can result in better and more robust recommender models. 

As the main contribution of this work, we propose an \textit{Adversarial Personalized Ranking} (APR) method to learn recommender models. With BPR as the building block, we introduce an additional objective function in APR to quantify the loss of a model under perturbations on its parameters. The formulation of APR can be seen as playing a minimax game, where the perturbations are optimized towards maximizing the BPR loss, and the model is trained to minimize both the BPR loss and the loss with adversarial perturbations. With a differentiable recommender model, the whole framework of APR can be optimized with the standard stochastic gradient descent. To demonstrate how it works, we derive the APR solver for MF and term the method as \textit{Adversarial Matrix Factorization} (AMF). We conduct extensive experiments on three public datasets constructed from Yelp, Pinterest and Gowalla that represent various item recommendation scenarios. The results justify the effectiveness of adversarial training for personalized ranking. Specifically, our AMF betters MF-BPR with a significant improvement over $11\%$ on average, outperforming the recently proposed neural recommender models~\cite{NCF,CDAE} and IRGAN~\cite{IRGAN}, and achieving state-of-the-art performance for item recommendation. 

%\cite{miyato2016adversarial}
%\cite{iCD}

%1. First work using adversarial training on pairwise loss. 

%reduce the sensitivity of the MF model to adversarial perturbations on the embeddings, and thus improve its generalization ability. 
% Paper structure
%SPACE
The reminder of the paper is organized as follows. We first present some background knowledge about MF and BPR, empirically showing that MF-BPR suffers from adversarial perturbations in Section~\ref{sec:preliminary}. We then elaborate our proposed APR learning framework and the AMF recommendation method in Section~\ref{sec:method}. We report experiment results in Section~\ref{sec:experiment}, before reviewing related work in Section~\ref{sec:related} and concluding the paper in Section~\ref{sec:conclusion}. 
